The Scaled Relative Graph of a Linear Operator

The scaled relative graph (SRG) of an operator is a subset of the complex plane. It captures several salient features of an operator, such as contractiveness, and can be used to reveal the geometric nature of many of the inequality based arguments used in the convergence analyses of fixed point iterations. In this paper we show that the SRG of a linear operator can be determined from the numerical range of a closely related linear operator. Furthermore we demonstrate that the SRG of a linear operator has a range of spectral and convexity properties, and satisfies an analogue of Hildebrant's theorem.

==> Maths.tex <==

\newcommand{\abs}[1]{\ensuremath{\left\vert#1\right\vert}}
\newcommand{\adj}[2][]{\ensuremath{\text{adj}_{{#1}}\left(#2\right)}}
\newcommand{\adjc}[2][]{\ensuremath{\text{adj}_{{#1}}\left[#2\right]}}
\newcommand{\Bdiagmatrix}[2]{\begin{bmatrix}
{#1}_{1}&&\\
&\ddots{}&\\
&&{#1}_{{#2}}
\end{bmatrix}}
\newcommand{\Beh}{\ensuremath{\mathcal{B}}}
\newcommand{\Blkmatrix}[3]{\begin{bmatrix}
{#1}_{11}&\cdots{}&{#1}_{1{#3}}\\
\vdots{}&\ddots{}&\vdots{}\\
{#1}_{{#2}1}&\cdots{}&{#1}_{{#2}{#3}}
\end{bmatrix}}
\newcommand{\cfunof}[1]{\ensuremath{\left\{#1\right\}}}
\newcommand{\Cont}{\ensuremath{\mathscr{C}_0}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\Cb}[1]{\ensuremath{\mathbb{C}\left[#1\right]}}
\newcommand{\cl}[1]{\ensuremath{\mathrm{cl}\,{#1}}}
\newcommand{\Ce}{\ensuremath{\mathbb{C}_{\infty}}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\diag}[1]{\ensuremath{\mathrm{diag}\left({#1}\right)}}
\newcommand{\disc}[1]{\ensuremath{\mathbb{D}\left({#1}\right)}}
\newcommand{\discc}[1]{\ensuremath{\overline{\mathbb{D}\left({#1}\right)}}}
\newcommand{\discalg}{\ensuremath{\mathscr{A}_0}}
\newcommand{\dom}[1]{\ensuremath{\mathrm{dom}\,{#1}}}
\newcommand{\eig}[1]{\ensuremath{\lambda\left(#1\right)}}
\newcommand{\ellipse}[1]{\ensuremath{\mathbb{E}\left(#1\right)}}
\newcommand{\funof}[1]{\ensuremath{\left(#1\right)}}
\newcommand{\F}{\ensuremath{\mathbb{F}}}
\newcommand{\graphof}[1]{\ensuremath{\mathbb{G}\left({#1}\right)}}
\newcommand{\graph}[1]{\ensuremath{\mathrm{gra}\,{#1}}}
\newcommand{\gdec}[1]{\ensuremath{\mathfrak{G}\left({#1}\right)}}
\newcommand{\hyper}[1]{\ensuremath{\mathscr{X}\left({#1}\right)}}
\newcommand{\hyperplane}[2]{\ensuremath{\mathit{l}\left(#1,#2\right)}}
\newcommand{\Htwo}{\ensuremath{\mathscr{L}_{2+}}}
\newcommand{\hilb}{\ensuremath{\mathcal{H}}}
\newcommand{\hinf}{\ensuremath{\mathscr{H}_\infty}}
\newcommand{\Hom}[1]{\ensuremath{\mathrm{Hom}\left(#1\right)}}
\newcommand{\hull}[1]{\ensuremath{\mathrm{co}\left(#1\right)}}
\newcommand{\hullbk}[1]{\ensuremath{\mathrm{co}_{\mathrm{Be\text{-}}\!\mathrm{Kl}}\left(#1\right)}}
\newcommand{\halfplane}[2]{\ensuremath{\mathbb{P}\left(#1,#2\right)}}
\newcommand{\herm}{\ensuremath{\mathbf{S}^n}}
\newcommand{\Hfty}{\ensuremath{\mathscr{H}_{\infty}}}
\newcommand{\HRule}{\rule{\linewidth}{0.5mm}}
\newcommand{\hvect}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\invgraph}[1]{\ensuremath{\overline{\mathscr{G}}_{#1}}}
\newcommand{\IQCt}[1]{\ensuremath{\text{IQC}\left(#1\right)}}
\newcommand{\IQC}[2]{\ensuremath{\sigma_{#1}\left(#2\right)}}
\newcommand{\IQCclass}[1]{\ensuremath{\mathbf{\Pi}_{#1}}}
\newcommand{\imag}[1]{\ensuremath{\mathrm{Im}\left(#1\right)}}
\newcommand{\inner}[2]{\ensuremath{\left\langle #1,#2\right\rangle}}
\newcommand{\jw}{\ensuremath{\left(j\omega\right)}}
\newcommand{\jwo}{\ensuremath{\left(j\omega_0\right)}}
\newcommand{\lft}[3]{\ensuremath{\mathcal{F}_{#1}\left({#2},{#3}\right)}}
\newcommand{\Lfty}{\ensuremath{\mathscr{L}_{\infty}}}
\newcommand{\Ltwor}{\ensuremath{\mathcal{L}^2\left(\mathbb{R}\right)}}
\newcommand{\Ltwo}{\ensuremath{\mathcal{L}^2\left(\mathbb{R}\right)}}
\newcommand{\Ltwob}[1]{\ensuremath{\mathscr{L}_{2\left[{#1}\right]}}}
\newcommand{\Ltwoe}[1][]{\ensuremath{\mathscr{L}_{2e}^{#1}}}
\newcommand{\Ltwoeb}[1]{\ensuremath{\mathscr{L}_{2e}\left[{#1}\right]}}
\newcommand{\Mn}{\ensuremath{\mathbf{M}^n}}
\newcommand{\nbyn}{\ensuremath{n\times n}}
\newcommand{\norm}[1]{\ensuremath{\left\Vert #1 \right\Vert}}
\newcommand{\ncomp}{\ensuremath{\text{$N$-component}}}
\newcommand{\nport}{\ensuremath{\text{$N$-port}}}
\newcommand{\proj}[2]{\ensuremath{\text{P}_{#1}\left(#2\right)}}
\newcommand{\possemidef}{\ensuremath{\mathbf{S}^n_{+}}}
\newcommand{\posdef}{\ensuremath{\mathbf{S}^n_{++}}}
\newcommand{\PR}{\ensuremath{\mathbf{PR}}}
\newcommand{\Rat}{\ensuremath{\mathscr{R}}}
\newcommand{\real}[1]{\ensuremath{\mathrm{Re}\left(#1\right)}}
\newcommand{\resolvent}[1]{\ensuremath{\rho\left(#1\right)}}
\newcommand{\RHardy}{\ensuremath{\mathscr{RH}_{\infty}}}
\newcommand{\RH}{\ensuremath{\mathscr{RH}_{\infty}}}
\newcommand{\RHb}[1]{\ensuremath{\mathbf{RH}_{\infty}\left[#1\right]}}
\newcommand{\RL}{\ensuremath{\mathbf{RL}_{\infty}}}
\newcommand{\RLb}[1]{\ensuremath{\mathbf{RL}_{\infty}\left[#1\right]}}
\newcommand{\RLfty}{\ensuremath{\mathscr{RL}_{\infty}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\RS}{\ensuremath{\mathbf{RS}_{\infty}}}
\newcommand{\Rb}[1]{\ensuremath{\mathbb{R}\left[#1\right]}}
\newcommand{\Rc}{\ensuremath{\overline{\R}_+}}
\newcommand{\select}[1]{\ensuremath{\textrm{E}\left(#1\right)}}
\newcommand{\selectsp}[1]{\ensuremath{\mathbb{E}\left(#1\right)}}
\newcommand{\sign}[1]{\ensuremath{\textrm{sign}\left(#1\right)}}
\newcommand{\SigIQC}[3]{\ensuremath{\Sigma{}\left(#1,#2,#3 \right)}}
\newcommand{\s}{\ensuremath{\left(s\right)}}
\newcommand{\sqfunof}[1]{\ensuremath{\left[#1\right]}}
\newcommand{\Shull}[1]{\ensuremath{\mathrm{S}\left(#1\right)}}
\newcommand{\SPR}{\ensuremath{\mathbf{SPR}}}
\newcommand{\spectrum}[1]{\ensuremath{\sigma\left(#1\right)}}
\newcommand{\srg}[1]{\ensuremath{\mathrm{SRG}\left(#1\right)}}
\newcommand{\srgc}[1]{\ensuremath{\mathrm{cl}\;\mathrm{SRG}\left(#1\right)}}
\newcommand{\srgh}[2]{\ensuremath{\mathrm{SRG}_{#2}\left(#1\right)}}
\newcommand{\srghc}[2]{\ensuremath{\mathrm{cl}\;\mathrm{SRG}_{#2}\left(#1\right)}}
\newcommand{\tm}{\ensuremath{\left(t\right)}}
\newcommand{\trunc}[1]{\ensuremath{\text{Q}_{#1}}}
\newcommand{\vect}[1]{\ensuremath{\mathrm{vec}\left(#1\right)}}
\newcommand{\vectr}[2]{\begin{bmatrix}
{#1}_{1}\\
\vdots{}\\
{#1}_{{#2}}
\end{bmatrix}}
\newcommand{\w}{\ensuremath{\left(\omega\right)}}
\newcommand{\wo}{\ensuremath{\left(\omega_0\right)}}
\newcommand{\W}[1]{\ensuremath{\mathrm{W}\left(#1\right)}}
\newcommand{\Wc}[1]{\ensuremath{\mathrm{cl}\;\mathrm{W}\left(#1\right)}}
\newcommand{\WH}[2]{\ensuremath{\mathrm{W}_{#2}\left(#1\right)}}
\newcommand{\wno}[1]{\ensuremath{\text{wno}\left({#1}\right)}}
\newcommand{\Z}[2]{\ensuremath{\mathbb{Z}_{[#1,#2]}}}


==> x.tex <==
\def \tikzexternallastkey {013B26D93A8B30AF57133EB6BF497BEA}%

